Secure Transmission of Sources over Noisy Channels with Side Information at the Receivers

This paper investigates the problem of source-channel coding for secure transmission with arbitrarily correlated side informations at both receivers. This scenario consists of an encoder (referred to as Alice) that wishes to compress a source and send it through a noisy channel to a legitimate receiver (referred to as Bob). In this context, Alice must simultaneously satisfy the desired requirements on the distortion level at Bob, and the equivocation rate at the eavesdropper (referred to as Eve). This setting can be seen as a generalization of the problems of secure source coding with (uncoded) side information at the decoders, and the wiretap channel. A general outer bound on the rate-distortion-equivocation region, as well as an inner bound based on a pure digital scheme, is derived for arbitrary channels and side informations. In some special cases of interest, it is proved that this digital scheme is optimal and that separation holds. However, it is also shown through a simple counterexample with a binary source that a pure analog scheme can outperform the digital one while being optimal. According to these observations and assuming matched bandwidth, a novel hybrid digital/analog scheme that aims to gather the advantages of both digital and analog ones is then presented. In the quadratic Gaussian setup when side information is only present at the eavesdropper, this strategy is proved to be optimal. Furthermore, it outperforms both digital and analog schemes, and cannot be achieved via time-sharing. By means of an appropriate coding, the presence of any statistical difference among the side informations, the channel noises, and the distortion at Bob can be fully exploited in terms of secrecy.

==> lastCase.tex <==

\begin{comment}
 
\clearpage
%------------------------------------------------------------------------------
\subsection{Last Case: $P_Y < P_Z$, $P_B > P_E$ -- Outer bound}

Let $(D,D_E)$ be an achievable tuple.
From the outer bound $\cR_\text{out}^P$, there exist random variables $U$, $V$, $Q$, $T$, $X$ with joint distribution $p(uvqtabexyz) = p(uv|a)p(abe)\,p(q|t)p(tx)p(y|x)p(z|y)$,\footnote{%
	Since it is assumed that $P_Y<P_Z$, according to Remark~\ref{rem:marginal}, the Markov chain $X\mkv Y\mkv Z$ can be assumed here without loss of generality.}
and a function $\hat A$, verifying
\begin{IEEEeqnarray*}{l}
I(V;A|B)\leq I(T;Y) 											\ ,\\
D 		\geq \bE\big[d(A,\hat A(V,B))\big] 						\ ,\\
\Delta	\leq  h(A|UE) - \Big[ I(V;A|B) - I(U;A|B) - 
					\Big( I(T;Y|Q) - I(T;Z|Q) \Big) \Big]_+ 	\ ,\\
\Var{X}  \leq P 												\ ,
\end{IEEEeqnarray*}
where $\Delta=\frac12\log(2\pi e\,D_E)$.

From the Markov chain $Q\mkv T\mkv X\mkv Y\mkv Z$, tuple $(D,\Delta)$ verifies the following inequalities:
\begin{IEEEeqnarray}{l}
I(V;A|B)\leq I(X;Y) 						\ ,\label{eq:gaussian:outer1}\\
D 		\geq \bE\big[d(A,\hat A(V,B))\big]	\ ,\label{eq:gaussian:outer2}\\
\Delta	\leq  h(A|UE) - \Big[ I(V;A|B) - I(U;A|B) - I(X;Y|Z) \Big]_+
											\ ,\label{eq:gaussian:outer3}\\
\Var{X} \leq P 								\ .\label{eq:gaussian:outer4}
\end{IEEEeqnarray}
Moreover, from the proof of Theorem~\ref{th:outer} (see \eqref{eq:outer:defU}, \eqref{eq:outer:defV} in Appendix~\ref{app:outer:proof}), we can restrict our attention to auxiliary variables $U$, $V$ s.t.\ $U\mkv V\mkv A\mkv E$ form a Markov chain.

We introduce two parameters:
$\nu = 2^{2h(A|VB)}/(2\pi e)$,
$\mu = 2^{2h(A|UB)}/(2\pi e)$.
From the fact that conditioning reduces the entropy and classical properties of the differential entropy, the above parameters are thus bounded as follows:
\begin{equation}
\label{eq:gaussian:outer:consnumu}
\nu \leq \mu \leq \frac1{1+\frac1{P_B}} \ .
\end{equation}

We now write \eqref{eq:gaussian:outer1}--\eqref{eq:gaussian:outer4} as functions of these parameters.
First, recalling that distortion measure $d$ is the Euclidean distance on $\bR$,
\begin{equation}
\label{eq:gaussian:outer:Dnu}
\bE\big[d(A,\hat A(V,B))\big] \geq \Var{A|VB} \geq \nu \ . 
\end{equation}

Since $P_B > P_E$, and according to Remark~\ref{rem:marginal}, we can assume that $A\mkv E\mkv B$ form a Markov chain.
In this case the side informations write:
\begin{IEEEeqnarray*}{rCL}
E &=& A + N_E							\ ,\\
B &=& A + N_E + \bar N_B = E + \bar N_B	\ ,
\end{IEEEeqnarray*}
where $\bar N_B\sim\cN(0,P_B-P_E)$ is independent of $A$ and $N_E\sim\cN(0,P_E)$.

Then, from the Markov chain $U\mkv A\mkv E\mkv B$, we write 
\begin{IEEEeqnarray*}{rCl}
\label{eq:gaussian:outer:hAUE}
h(A|UE)	&=& h(A|UBE) 					\\
		&=& h(A|UB) - I(A;E|UB) 		\\
		&=& h(A|UB) - h(E|UB) + h(E|AB) \ .
\end{IEEEeqnarray*}

Now, in order to find an upper bound on the latter quantity, we need the following expansion of $E$, for any $\gamma\in\bR$:
\[
E = \gamma B + (1-\gamma) A + C \ ,
\]
where
\[
C = (1-\gamma)N_E - \gamma \bar N_B \ .
\]
Note that $(A,B,C)$ is a Gaussian vector, and that $A$ and $C$ are independent for any $\gamma$.
The usefulness of the above expansion comes from the fact that $C$ is also independent of $B$ if $\gamma=\frac{P_E}{P_B}$:
\begin{IEEEeqnarray*}{rCL}
\bE[BC]	&=& (1-\gamma)\,\bE\left[ B N_E \right] - \gamma\,\bE\left[ B \bar N_B \right]	\\
		&=& (1-\gamma)P_E - \gamma\,(P_B-P_E)	\\
		&=& P_E - \gamma P_B					\\
		&=& 0									\ .
\end{IEEEeqnarray*}
Finally, since $U$ only depends on $A$, $C$ is independent of $(U,A,B)$.

Using the above expansion, we can write 
\begin{IEEEeqnarray*}{rCl}
h(E|UB)	&=& h(\gamma B + (1-\gamma) A + C|UB)	\\
		&=& h((1-\gamma) A + C|UB)				\ .
\end{IEEEeqnarray*}
And from the above paragraph, the conditional EPI holds between $A$ and $C$ (given $(U,E)$):
\begin{equation}
\label{eq:gaussian:outer:condEPI}
2^{2h((1-\gamma) A + C|UB)}
	\geq 2^{2h((1-\gamma) A|UB)} + 2^{2h(C|UB)} \ .
\end{equation}
The last entropy can be lower bounded as follows:
\begin{IEEEeqnarray*}{rCL}
h(C|UB)	&=& 	h((1-\gamma)N_E - \gamma \bar N_B | UB)	\\
		&\geq&	h((1-\gamma)N_E - \gamma \bar N_B | AB)	\\
		&=&		h(E|AB)								\ .
\end{IEEEeqnarray*}

Gathering \eqref{eq:gaussian:outer:hAUE} and \eqref{eq:gaussian:outer:condEPI}, we obtain:
\begin{IEEEeqnarray*}{rCl}
\label{eq:gaussian:outer:hAUEmu}
h(A|UE)	&\leq&	h(A|UB) - \frac12\log\left( (1-\gamma)^2\,2^{2 h(A|UB)} + 2^{2 h(E|AB)} \right) + h(E|AB)	\\
		&=&		\frac12\log\left( \frac1{\frac1{2^{2 h(A|UB)}} + \frac{(1-\gamma)^2}{2^{2 h(E|AB)}}} \right) \\
		&=&		\frac12\log\left( \frac{2\pi e}{\frac1\mu + \frac{\left(1-\frac{P_E}{P_B}\right)^2}{P_E\left(1-\frac{P_E}{P_B}\right)}} \right)	\\
		&=&		\frac12\log\left( \frac{2\pi e}{\frac1\mu + \frac1{P_E} - \frac1{P_B} } \right)
				\yesnumber\ .
\end{IEEEeqnarray*}

From the Markov chain $X\mkv Y\mkv Z$, there exists a random variable $\widetilde N_Z\sim\cN(0,P_Z-P_Y)$, independent of $Y$ such that $Z = Y + \widetilde N_Z$. 
Then the EPI~\cite{shannon1948mathematical,elgamal2010lecture} yields:
\[
2^{2 h(Z)} \geq 2^{2 h(Y)} + 2^{2 h(\widetilde N_Z)}	\ .
\]
From the latter equation and inequality $\Var{Y}\leq P+P_Y$,
\begin{IEEEeqnarray*}{rCl}
\label{eq:gaussian:outer:IXYZzeta}
I(X;Y|Z)	&=&		h(Y) - h(Y|X) - h(Z) + h(Z|X)						\\
			&\leq&	h(Y) - h(N_Y) - \frac12\log\left( 2^{2 h(Y)} 
						+ 2^{2 h(\widetilde N_Z)} \right) + h(N_Z)		\\		
			&\leq&	\frac12\log\left( \frac1{ 1 + \frac{P_Z-P_Y}{P+P_Y}}\,
									  \frac{P_Z}{P_Y} \right)			\\	
			&=&		\frac12\log\left( \frac{1+\frac{P}{P_Y}}
										{1+\frac{P}{P_Z}} \right)		\ .\yesnumber
\end{IEEEeqnarray*}

Gathering the above equations, tuple $(D,D_E)$ verifies the following inequalities:
\begin{IEEEeqnarray*}{l}	
\nu \leq \mu \leq \frac1{1+\frac1{P_B}}								\ ,\\
 \frac1{1+\frac1{P_B}}\,\frac1\nu	\leq 1 + \frac{P}{P_Y} 			\ ,\\
D			\geq \nu			 									\ ,\\
D_E			\leq \frac1{\frac1\mu + \frac1{P_E} - \frac1{P_B}}		\ ,\\
D_E			\leq \frac1{\frac1\mu + \frac1{P_E} - \frac1{P_B}}\,\frac\nu\mu\,
						\frac{1+\frac{P}{P_Y}}{1+\frac{P}{P_Z}}		\ .
\end{IEEEeqnarray*}

Eliminating parameter $\nu$ and $\mu$ yields the result shown in the table of the next page.

\begin{comment}
\begin{landscape}
%------------------------------------------------------------------------------
\subsection{General Case--Summary}

We can eventually prove the following closed-form expressions:

\begin{center}
\begin{IEEEeqnarraybox}[\IEEEeqnarraystrutmode\IEEEeqnarraystrutsizeadd{15pt}{5pt}]{x/c/V/l/v/l/v/l/x}
&				&&	A\mkv B\mkv E\ (P_B\leq P_E)
					&& A\mkv E\mkv B\ (P_B>P_E)
						&& B=\emptyset\ (P_B\to\infty) \\
\IEEEeqnarrayrulerow\\
&X\mkv Y\mkv Z	&& D	\geq \frac1{1+\frac1{P_B}}\cdot\frac1{1+\frac{P}{P_Y}}
					&& D	\geq \frac1{1+\frac1{P_B}}\cdot\frac1{1+\frac{P}{P_Y}}
						&& D	\geq \frac1{1+\frac{P}{P_Y}} \\
&(P_Y<P_Z)		&& D_E	\leq \frac1{1+\frac1{P_E}}
					&& D_E	\leq \frac1{1+\frac1{P_E}}
						&& D_E	\leq \frac1{1+\frac1{P_E}} \\
&				&& D_E	\leq D\cdot\frac{1+\frac1{P_B}}{1+\frac1{P_E}}\cdot\frac{1+\frac{P}{P_Y}}{1+\frac{P}{P_Z}}
					&& D_E	\leq \frac1{\frac1D\cdot\frac{1+\frac{P}{P_Z}}{1+\frac{P}{P_Y}}+\frac1{P_E}-\frac1{P_B}}
						&& D_E	\leq \frac1{\frac1D\cdot\frac{1+\frac{P}{P_Z}}{1+\frac{P}{P_Y}}+\frac1{P_E}} \\
&				&& \text{Digital scheme (optimal)}
					&& \text{Outer bound}
						&& \text{Hybrid scheme (optimal)} & \\
\IEEEeqnarrayrulerow\\
&X\mkv Z\mkv Y	&& D	\geq \frac1{1+\frac1{P_B}}\cdot\frac1{1+\frac{P}{P_Y}}
					&& D	\geq \frac1{1+\frac1{P_B}}\cdot\frac1{1+\frac{P}{P_Y}}	\\
&(P_Y\geq P_Z)	&& D_E	\leq \frac1{1+\frac1{P_E}}
					&& D_E	\leq \frac1{1+\frac1{P_E}}	\\
&				&& D_E	\leq D\cdot\frac{1+\frac1{P_B}}{1+\frac1{P_E}}
					&& D_E	\leq \frac1{\frac1D+\frac1{P_E}-\frac1{P_B}} \\
&				&& \text{Digital scheme (optimal)}
					&& \text{Digital scheme (optimal)}
\end{IEEEeqnarraybox}
\end{center}
\end{landscape}

\clearpage
\end{comment}
